Statistics of the Effective Massive MIMO Channel in Correlated Rician Fading

Massive MIMO base stations use multiple spatial diversity branches, which are often assumed to be uncorrelated in theoretical work. Correlated branches are considered seldom since they are mathematically less tractable. For correlated Rician fading, only the first- and second-order moments have been explored. To describe propagation environments more accurately, full distribution functions are needed. This manuscript provides these functions for the maximum ratio combining effective channel, a quadratic form of a random complex normal channel vector. Its mean vector and covariance matrix are based on a plane wave model incorporating array geometry, antenna element pattern, power angular spectra and power delay profiles. Closed-form approximations of the distribution functions are presented, to allow the fast evaluation of many real-world scenarios. The statistical framework is used to show that low-directivity antenna elements provide better performance in angular constricted Rician fading with off-axis incidence than high-directivity elements. Moreover, two base station array layouts are compared, showing that a half-circle array illuminates a cell more evenly than a uniform linear array. With the full distribution functions available, performance can be compared over the full range of received powers and not only based on the average SNR.

==> measurements.tex <==
\section{Measurements}

\subsection{Empiric}
There exists a dataset of indoor massive \gls{mimo} channels with high resolution sampling of the coverage area of a room at KU Leuven \cite{de-bast_ku_leuven_csi_2020}. 
They have recorded a quasi-static channel over \SI{20}{\mega\hertz} (100 sub-carriers) with center frequency \SI{2.61}{\mega\hertz} between a \gls{bs} with 64 antennas and 252004 potential user positions distributed over four squares of \SI{1.25}{\meter} by \SI{1.25}{\meter} each.
The \gls{bs} antennas are grouped into \glspl{ula} of 8 elements, which allowed them to record different configurations: a 64 element \gls{ula} along one side of the room, a 8 times 8 \gls{ura} at the center of the same side and a distributed configuration of 8 \glspl{ula} arranged in a circular fashion.
All configurations have been used for \gls{los} measurements.
Additionally, the room was modified for the \gls{ura} configuration to shape a \gls{nlos} channel.

\begin{figure}
	\centering
	\input{tikz/ku_leuven_geometry.tikz}
	\caption{Locations of the local regions with respect to the array configurations.}
	\label{fig:geometry}
\end{figure}

==> spherical_harmonics.tex <==
\subsubsection{Unnormalized Complex Spherical Harmonic Coefficients}

The unnormalized complex spherical harmonic coefficients $S^m_l$ arrive from expanding the angular function $p(\theta,\phi)$ with spherical harmonics:
\begin{equation}
    S^m_l = \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \overline{Y}^m_l(\theta, \phi) \cos \phi\;d\phi\,d\theta
\end{equation}
\todo{write definitions down to get to the normalised version of $\overline{Y}^m_l(\theta, \phi)$ complex spherical harmonics}

\begin{align}
    S_0^0 &= \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \cos \phi\;d\phi\,d\theta \\
    S_1^0 &= \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \sin \phi \cos \phi\;d\phi\,d\theta \\
    S_1^1 &= \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \cos \phi\;\mathrm{e}^{j\theta} \cos \phi \;d\phi\,d\theta \\
    S_0^2 &= \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \left(\sin^2 \phi - \frac{1}{3} \right) \cos \phi \;d\phi\,d\theta \\
    S_1^2 &= \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \cos \phi \sin \phi \mathrm{e}^{j\theta} \cos \phi \;d\phi\,d\theta \\
    S_2^2 &= \int_0^{2\pi} \int_{-\frac{\pi}{2}}^{\frac{\pi}{2}} p(\theta,\phi) \cos^2 \phi \mathrm{e}^{j 2 \theta} \cos \phi \;d\phi\,d\theta
\end{align}
